An Empirical Survey of Data Augmentation for Limited Data Learning in NLP

NLP has achieved great progress in the past decade through the use of neural models and large labeled datasets. The dependence on abundant data prevents NLP models from being applied to low-resource settings or novel tasks where significant time, money, or expertise is required to label massive amounts of textual data. Recently, data augmentation methods have been explored as a means of improving data efficiency in NLP. To date, there has been no systematic empirical overview of data augmentation for NLP in the limited labeled data setting, making it difficult to understand which methods work in which settings. In this paper, we provide an empirical survey of recent progress on data augmentation for NLP in the limited labeled data setting, summarizing the landscape of methods (including token-level augmentations, sentence-level augmentations, adversarial augmentations, and hidden-space augmentations) and carrying out experiments on 11 datasets covering topics/news classification, inference tasks, paraphrasing tasks, and single-sentence tasks. Based on the results, we draw several conclusions to help practitioners choose appropriate augmentations in different settings and discuss the current challenges and future directions for limited data learning in NLP.

==> ACL 2021 - Survey Data Augmentation (1)/glue_10.tex <==
% GLUE
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\renewcommand{\tabcolsep}{5pt}
\begin{tabular}{cccccccccc} \toprule
&\multirow{2}{*}{\textbf{Methods}}                                                                        & \multirow{2}{*}{\textbf{Types}}  & \multicolumn{3}{c}{\textbf{Inference}} & \multicolumn{2}{c}{\textbf{Paraphrase}} & \multicolumn{2}{c}{\textbf{Single Sentence}} \\ %\cmidrule{4-10} 
\cmidrule(lr){4-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}
& &  & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE}  & \textbf{QQP}  & \textbf{MRPC} & \textbf{SST-2} & \textbf{CoLA}\\ \midrule


&\multirow{1}{*}{None} & -    & 35.2(0.7)	& 51.8(7.0)	& 49.8(3.1)	& 63.9(9.1)	& 61.8(21.2)& 	60.5(13.1)	& 12.9(6.32)  \\  \cmidrule(lr){2-10} %\cmidrule(lr){4-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}
                                                                                                                                                                
&\multirow{1}{*}{SR}   & \multirow{6}{*}{Token} &35.1(2.3)	&51.4(7.2) &	51.5(3.4)	&61.3(9.7)	&59.7(26.3)	&62.1(17.4)	&7.2(11.6)      \\
                                                                                
&\multirow{1}{*}{LM}     &     &35.3(0.8)	&51.0(8.0)	&49.0(1.4)	&62.4(11)	&61.0(24.3)	&62.8(9.8)	&6.8(15.8)    
                                                                                   \\ \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Supervised}}}}
&\multirow{1}{*}{RI}     &     &34.9(2.6)	&51.5(8.4)	&\textbf{51.5(1.4)}	&60.6(10.9)	&60.6(25.0)	&63.3(12.2)	&7.8(7.42)      
                                                                                 \\ 
&\multirow{1}{*}{RD}       &    &\textbf{35.5(2.1)}	&51.1(8.4)	&50.9(2.4)	&62.4(11.3)	&61.2(22.0)	&59.7(18.4)	&7.1(16.6)      
                                                                                  \\ 
&\multirow{1}{*}{RS}       &      &35.1(1.1)	 &51.5(7.0)	 &50.9(5.0)	 &\textbf{62.6(6.7)}	 &\textbf{63.2(22.5)}	 &61.2(10.8)	 &5.2(17.0)    
                                                                                \\ 
&\multirow{1}{*}{WR}     &    &34.5(2.6)	&\textbf{52.0(3.8)}	&50.0(0.9)	&60.6(10.2)	&61.0(25.3)	&61.8(12.5)	&7.0(10.6)       
                                                                                  \\ \cmidrule(lr){2-10}

&\multirow{1}{*}{RT} & Sentence &   35.3(0.5)	&51.1(9.6)	&50.8(4.4)	&60.5(17.8)	&61.8(23.7)	&62.0(1.99)	&8.37(8.35)    
                                                                                   \\ \cmidrule(lr){2-10}
                                                                                   
&\multirow{1}{*}{ADV} & \multirow{3}{*}{Hidden}    &33.3(4.7)	&49.7(1.8)	&48.3(12.1)	&57.5(24.7)	&61.5(21.5)	&53.3(13.07)	&1.37(4.66)     
                                                                                   \\ 
                                                                                   
                                                                                   


&\multirow{1}{*}{Cutoff} &     &35.1(2.3)	&51.4(8.3)	&52.2(3.6)	&62.6(8.8)	&61.0(21.2)	&\textbf{63.5(8.45)}	&\textbf{12.4(9.58)}   \\  

&\multirow{1}{*}{Mixup} &        &32.6(3.5)	 &49.9(1.4)	 &49.8(9.2)	 &63.0(0.3)	 &62.1(19.8)	 &62.3(12.3)	 &4.03(8.68)  
                                                                                    
                                                                                 \\ \midrule \midrule
                                                                                   
                                                                                


&\multirow{1}{*}{SR}   & \multirow{6}{*}{Token}    & 35.6(1.0)	&52.1(4.5)	&\textbf{52.9(5.4)}	&53.5(10.7)	&68.1(4.0)	&61.8(37.9)	&6.65(5.69)     \\ \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Semi-Supervised}}}}
                                                                                
&\multirow{1}{*}{LM}     &    &35.0(3.3)	&52.5(4.2)	&50.2(6.5)	&47.9(34.1)	&68.4(3.8)	&57.3(14.2)	&6.38(6.3)
                                                                                   \\ 
&\multirow{1}{*}{RI}     &    &\textbf{35.8(1.7)}	&52.1(4.1)	&50.7(1.4)	&59.6(5.1)	&64.9(8.9)	&58.3(14.8)	&6.55(0.91)
                                                                                 \\ 
&\multirow{1}{*}{RD}       &   &35.2(0.5)	&52.1(5.2)	&52.6(4.9)	&56.1(16.0)	&62.4(30.6)	&55.7(16.4)	&4.33(10.9)
                                                                                  \\ 
&\multirow{1}{*}{RS}       &     &34.6(2.5)	&52.1(6.2)	&51.5(3.7)	&49.8(7.9)	&63.2(22.5)	&55.2(15.3)	&7.77(11.77)   
                                                                                \\ 
&\multirow{1}{*}{WR}     &    &34.8(2.5)	&52.1(4.1)	&50.9(1.8)	&51.8(16.0)	&63.1(23.5)	&54.8(13.8)	&5.43(17.8)
                                                                                  \\ \cmidrule(lr){2-10}

&\multirow{1}{*}{RT} & Sentence  &35.3(2.7)	&\textbf{52.7(4.8)}	&51.6(4.1)	&\textbf{63.9(7.5)}	&62.2(12.5)	&\textbf{61.9(20.8)}	&\textbf{11.6(14.5)}
                                                                                   \\ \cmidrule(lr){2-10}
                                                                                   
&\multirow{1}{*}{ADV} & \multirow{2}{*}{Hidden}   &36.2(8.9)	&50.6(1.9)	&50.9(6.8)	&59.1(14.7)	&63.9(9.1)	&53.1(5.0)	&7.64(25.1)     
                                                                                   \\ 
                                                                                   
                                                                                   


&\multirow{1}{*}{Cutoff} &   &35.3(2.8)	&52.5(4.3)	&51.7(6.5)	&62.9(9.9)	&\textbf{68.6(4.4)}	&54.3(9.8)	&4.11(11.8)
                                                                                 \\ \bottomrule 

\end{tabular}
\caption{\small GLUE results with 10 labeled examples per class. We report the average results across 3 different random seeds with the 95\% confidence interval and \textbf{bold} the best results.} \label{Tab:Glue_10}
\end{table*}

==> ACL 2021 - Survey Data Augmentation (1)/glue_100.tex <==
% GLUE
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\renewcommand{\tabcolsep}{5pt}
\begin{tabular}{cccccccccc} \toprule
&\multirow{2}{*}{\textbf{Methods}}                                                                        & \multirow{2}{*}{\textbf{Types}}  & \multicolumn{3}{c}{\textbf{Inference}} & \multicolumn{2}{c}{\textbf{Paraphrase}} & \multicolumn{2}{c}{\textbf{Single Sentence}} \\ \cmidrule(lr){4-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}
& &  & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE}  & \textbf{QQP}  & \textbf{MRPC} & \textbf{SST-2} & \textbf{CoLA}\\ \midrule


&\multirow{1}{*}{None} & -    &45.0(6.9)	&63.2(10.7)	&59.9(3.1)	&71.0(2.6)	&68.1(7.4)	&82.7(4.0)	&28.7(9.5)  \\\cmidrule(lr){2-10}
                                                                                                                                                                
&\multirow{1}{*}{SR}   & \multirow{6}{*}{Token} &44.6(7.2)	&62.9(9.4)	&61.0(10.0)	&68.9(2.2)	&66.7(4.4)	&84.0(1.9)	&24.6(5.1)     \\
                                                                                
&\multirow{1}{*}{LM}     &     &45.4(6.2)	&60.6(7.7)	&\textbf{61.5(9.1)}	&69.6(1.7)	&67.2(2.8)	&83.8(3.1)	&18.5(9.7)
                                                                                   \\ \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Supervised}}}}
&\multirow{1}{*}{RI}     &     &\textbf{45.8(7.5)}	&\textbf{64.2(10.7)}	&60.0(11.3)	&69.2(0.6)	&69.1(4.8)	&84.3(1.4)	&27.3(19.9)
                                                                                 \\ 
&\multirow{1}{*}{RD}       &    &43.7(8.4)	&63.6(9.4)	&59.2(9.0)	&69.2(1.5)	&69.2(5.5)	&82.3(2.05)	&20.2(21.5)
                                                                                  \\ 
&\multirow{1}{*}{RS}       &     &42.4(6.2)	&63.3(9.1)	&57.8(11.9)	&68.3(1.6)	&69.0(3.4)	&82.5(5.0)	&24.3(20.8)    
                                                                                \\ 
&\multirow{1}{*}{WR}     &    &44.6(6.3)	&61.6(8.8)	&57.8(9.3)	&66.7(1.8)	&66.9(6.4)	&83.5(1.9)	&17.7(23.3)
                                                                                  \\\cmidrule(lr){2-10}

&\multirow{1}{*}{RT} & Sentence &44.8(7.8)	&59.0(7.6)	&60.4(5.7)	&\textbf{69.9(4.0)}	&\textbf{69.6(1.6)}	&84.3(3.27)	&19.2(7.63)
                                                                                   \\ \cmidrule(lr){2-10}
                                                                                   
&\multirow{1}{*}{ADV} & \multirow{3}{*}{Hidden}    &39.1(10.9)	&50.1(3.1)	&57.3(8.7)	&63.7(1.9)	&68.7 (6.3)	&69.8(5.3)	&16.5(9.2)
                                                                                   \\ 
                                                                                   
                                                                                   


&\multirow{1}{*}{Cutoff} &     &44.9(5.5)	&63.0(10.2)	&59.3(8.8)	&69.9(0.7)	&66.5(1.3)	&\textbf{84.7(0.9)}	&\textbf{26.0(16.3)}   \\  

&\multirow{1}{*}{Mixup} &        &35.7(7.3)	&51.4(4.4)	&60.5(6.52)	&64.5(5.4)	&67.9 (7.1)	&83.5(3.4)	&20.1(18.8)
                                                                                    
                                                                                 \\ \midrule  \midrule 
                                                                                   
                                                                                


&\multirow{1}{*}{SR}   & \multirow{6}{*}{Token}    &42.9(7.3)	&60.1(6.2)	&58.5(9.7)	&65.0(6.0)	&67.6(3.1)	&85.1(3.5)	&18.9(6.7)  \\ \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Semi-Supervised}}}}
                                                                                
&\multirow{1}{*}{LM}     &   &43.7(4.5)	&60.9(10.4)	&56.9(8.3)	&59.3(12.0)	&70.0(4.4)	&83.9(4.1)	&21.7(6.8)
                                                                                   \\ 
&\multirow{1}{*}{RI}     &    &44.7(4.6)	&62.5(10.5)	&56.0(6.3)	&68.3(0.1)	&67.0(3.9)	&84.2(3.0)	&23.0(10.3)
                                                                                 \\ 
&\multirow{1}{*}{RD}       &   &41.4(2.9)	&59.4(6.4)	&56(0.0)	&\textbf{69.3(2.8)}	&70.4(7.4)	&83.6(2.3)	&13.1(6.1)
                                                                                  \\ 
&\multirow{1}{*}{RS}       &     &40.3(2.0)	&60.3(8.7)	&56.4(11.6)	&66.8(2.3)	&69.0(3.4)	&84.5(3.6)	&19.4(2.7)
                                                                                \\ 
&\multirow{1}{*}{WR}     &   &43.9(3.1)	&60.5(8.8)	&56.3(7.1)	&65.4(4.3)	&67.2(2.1)	&83.3(4.5)	&16.9(6.2)
                                                                                  \\ \cmidrule(lr){2-10}

&\multirow{1}{*}{RT} & Sentence   & \textbf{45.4(7.7)}	 & \textbf{63.8(5.0)}	 & \textbf{59.9(9.1)}	 & 68.3(2.9)	 & 67.5(0.7)	 & \textbf{83.9(1.7)}	 & 20.4(3.6)                         \\ \cmidrule(lr){2-10}
                                                                                   
&\multirow{1}{*}{ADV} & \multirow{2}{*}{Hidden}   &44.1(3.4)	&58.1(4.0)	&58.6(5.2)	&63.0(10.8)	&67.6(5.2)	&80.0(7.3)	&13.5(7.8)
                                                                                   \\ 
                                                                                   
                                                                                   


&\multirow{1}{*}{Cutoff} &    &42.7(4.2)	 &60.3(7.4)	 &57.9(12.6)	 &67.2(4.4)	 &\textbf{71.4(2.0)}	 &82.5(5.4)	 &\textbf{23.9(2.7)}
                                                                                 \\ \bottomrule 

\end{tabular}
\caption{\small GLUE results with 100 labeled examples per class. We report the average results across 3 different random seeds with the 95\% confidence interval and \textbf{bold} the best results.} \label{Tab:Glue_100}
\end{table*}

==> ACL 2021 - Survey Data Augmentation (1)/rte_examples.tex <==
\begin{table*}
\begin{tabular}{p{0.3\linewidth} p{0.3\linewidth} p{0.3\linewidth} } \toprule
\textbf{Original}  & \textbf{Cutoff (Best)} & \textbf{Language Model (Worst)} \\ 
\midrule
\midrule
Sentence 1: The Walt Disney Co. donated one of the world's most significant private collections of African artwork, yesterday, to the Smithsonian's National Museum of African Art. & Sentence 1: The Walt Disney Co. donated one of the world's most significant private collections of African artwork, yesterday, to the Smithsonian's National Museum of African one & Sentence 1: The Walt Disney Co. donated one of the world's most significant private collections of African artwork [PAD] [PAD] [PAD] to the Smithsonian's National Museum of African Art. \\
Sentence 2: Disney gave the Smithsonian a trove of sought-after African art. & Sentence 2: Disney gave the Smithsonian a trove of south African art. & Sentence 2: Disney gave the Smithsonian a trove of [PAD] African art. \\
\midrule
Entailment & Entailment & Not Entailment \\
\midrule
\midrule


Sentence 1: An explosion, followed by a raging fire, demolished a plastics factory, killing at least three people and injuring at least 37. & Sentence 1: An explosion, followed by a raging fire, demolished a the factory, killing at least three people and injuring at least 37. & Sentence 1: An explosion, followed by [PAD] [PAD] fire, demolished a plastics factory, killing at least three people and injuring at least 37. \\
Sentence 2: A massive blast at a plastics factory killed at least two people. & Sentence 2: A massive blast at a plastics factory killed at shot two people. & Sentence 2: A massive blast at a plastics [PAD] killed at least two people. \\
\midrule 
Entailment & Entailment & Not Entailment \\
\midrule
\midrule

Sentence 1: The prize is named after Alfred Nobel, a pacifist and entrepreneur who invented dynamite in 1866. Nobel left much of his wealth to establish the award, which has honoured achievements in physics, chemistry, medicine, literature and efforts to promote peace since 1901. & Setence 1: The prize is named after Alfred Nobel, a pacifist and entrepreneur who invented dynamite in 1866. Nobel left much of his wealth to establish the nobel which has honoured achievements in physics, chemistry, medicine, literature and efforts to promote peace since 1901. & The prize is named after Alfred Nobel, a pacifist and entrepreneur who invented dynamite in 1866 . Nobel left much of his wealth [PAD] [PAD] [PAD] [PAD], which has honoured achievements in physics, chemistry, medicine, literature and efforts to promote peace since 1901. \\
\midrule 
Sentence 2: Alfred Nobel invented dynamite in 1866. & Sentence 2: Alfred Nobel invented dynamite in 1866. & Sentence 2: Alfred Nobel invented dynamite in 1866. \\
\midrule
Entailment & Entailment & Not Entailment \\ \bottomrule 


% 
\end{tabular}
\caption{Examples of different data augmentation methods on RTE and whether they preserve the original label or not}
\label{Tab:rte_ex}
\end{table*}

==> ACL 2021 - Survey Data Augmentation (1)/tc_10.tex <==
\begin{table*}[t]
%\small
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{ccccccc} \toprule
& \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Types}} & \multicolumn{2}{c}{\textbf{News Classification}} & \multicolumn{2}{c}{\textbf{Topic Classification}} \\\cmidrule(lr){4-5}\cmidrule(lr){6-7} 
& &  &  \textbf{AG News} & \textbf{20 Newsgroup} & \textbf{Yahoo Answers} & \textbf{PubMed} \\ \midrule
& None  & - & 78.8(8.9) & 65.2(4.8) & 56.6(9.4) & 63.7(6.1)/49.3(3.9) \\ \cmidrule(lr){2-7}
& SR &   & 79.4(5.9) & 66.1(2.5) & 56.0(10.1) & 62.4(5.7)/48.3(3.9) \\ 
& LM & \multirow{4}{*}{Token}   & 76.8(5.1) & 60.0(14.4) & 56.2(8.4) & 60.9(3.0)/47.4(2.5)  \\ 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Supervised}}}}
 & RI &  & 79.5(4.9) & 66.6(0.6) & 57.3(12.0) & 63.7(4.2)/49.4(2.1) \\ 
& RD &  & 79.6(5.0) & 66.8(3.0) & 58.0(8.3)  & 63.4(5.0)/49.3(1.5)  \\ 
& RS &  & 79.5(5.3) & 64.8(10.8) & 57.1(10.3) & 63.8(7.4)/49.5(3.3) \\ 
& WR &  & 79.7(2.0) & \textbf{67.5(4.2)} & \textbf{59.3(8.9)} & \textbf{64.9(4.9)/49.4(2.5)} \\ \cmidrule(lr){2-7}
& RT & Sentence & \textbf{80.1(4.3)} & 65.1(7.9) & 57.1(9.6) & 60.2(5.1)/46.3(6.4) \\ \cmidrule(lr){2-7}
& ADV &  \multirow{3}{*}{Hidden}  & 78.2 (5.3) & 65.5(1.6) & 53.8(4.89) & 37.4(2.6)/19.9(10.6) \\
& Cutoff & & 79.3(5.0) & 66.6(1.4) & 57.3(9.3) & 60.5(8.3)/46.6(9.4)  \\
& Mixup &  & 80.0 (6.52) & 65.9(3.1) & 57.8(4.19) & 51.4(19.3)/39.8(3.2) \\
\midrule \midrule
& SR & \multirow{5}{*}{Token}   & 69.6(29.3) & 65.7(1.8) & 51.4(9.4) & 59.3(5.9)/43.1(11.9)  \\ 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Semi Supervised}}}} & LM &   & 68.5(13.7) & 68.3(2.1) & 53.2(6.3) & 61.5(6.6)/46.4(4.4)  \\ 
 & RI &  & 65.8(5.5) & 66.7(1.1) & 50.5(3.2) & 61.4(11.3)/44.4(17.4)  \\ 
& RD &  & 73.2(14.0) & 66.1(3.3) & 51.5(7.5) & 59.3(7.1)/46.0(3.8) \\ 
 & RS &  & 71.6(16.6) & 65.0(2.0) & 51.1(7.1) & 64.2(12.1)/46.7(11.5)  \\ 
& WR &  & 74.1(12.3) & \textbf{69.3(2.5)} & 55.6(5.9) & 60.4(7.5)/43.7(14.2) \\ \cmidrule(lr){2-7}
& RT & Sentence & 82.1(8.2) & 68.8(2.4) & 59.8(3.9) & \textbf{64.3(1.2)/49.8(1.9)}\\  \cmidrule(lr){2-7}
& ADV & \multirow{2}{*}{Hidden}  & \textbf{82.3(2.33)} & 66.8(5.9) & 55.9(3.89) & 62.2(10.8)/46.2(9.8) \\ 
& Cutoff &  & 79.9(5.5) & 67.9(0.8) & \textbf{60.1(1.0)} & 62.7(9.0)/48.1(3.2) \\ 
\bottomrule 
\end{tabular}}
\caption{\small Topic Classification and News Classification results with 10 examples. We report the average results across 3 different random seeds with the 95\% confidence interval and \textbf{bold} the best results.. For PubMed, we report the accuracy and F1 score. } \label{Tab:Cls}
\end{table*}

==> ACL 2021 - Survey Data Augmentation (1)/tc_100.tex <==
\begin{table*}[t]
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{ccccccc} \toprule
& \multirow{2}{*}{\textbf{Methods}} & \textbf{Types} & \multicolumn{2}{c}{\textbf{News Classification}} & \multicolumn{2}{c}{\textbf{Topic Classification}} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7} 
& & - &  \textbf{AG News} & \textbf{20 Newsgroup} & \textbf{Yahoo Answers} & \textbf{PubMed} \\ \midrule 
& None  & - & 87.9(1.05) & 79.5(0.3) & 68.6(0.71) & 75.2(1.5)/59.5(2.0)  \\ \cmidrule(lr){2-7}
& SR &  & 88.5(0.87) & 80.0(2.2) & \textbf{69.7(1.62)} & 76.5(1.0)/60.7(0.7) \\ 
& LM & \multirow{4}{*}{Token}  & 88.1(1.00) & \textbf{80.5(1.8)} & 68.8(3.2) & 75.8(2.5)/59.9(1.7) \\ 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Supervised}}}}
 & RI &  & 88.0(2.08) & 80.1(3.1) & 69.1(1.68) & 76.2(2.9)/60.3(1.7) \\ 
& RD &  & 88.1(0.84) & 80.2(2.9) & 68.7(2.2) & \textbf{76.9(0.6)/60.9(0.6)}  \\ 
& RS &  & 88.4(0.97) & 79.5(2.1) & 69.0(2.03) & 76.6(0.2)/60.6(0.7) \\ 
& WR &  & 87.9(1.19) & 79.3(2.5) & 69.4(5.89) & 76.4(1.8)/60.4(1.6)\\ \cmidrule(lr){2-7}
& RT & Sentence & 88.3(0.17) & 80.4(0.7) & 68.8(1.88) & 76.1(0.5)/60.3(0.5) \\ \cmidrule(lr){2-7}
& ADV &  \multirow{3}{*}{Hidden} & 87.6(0.33) & 78.5(1.4) & 67.4(0.74) & 75.6(4.0)/59.8(3.5) \\
& Cutoff & & 88.3(0.38) & 79.8(1.0) & 68.7(0.47) & 75.9(1.3)/60.1(0.7)  \\
& Mixup &  & \textbf{88.6(1.31)} & {80.5(3.4)} & 68.27(1.76) & 74.8(1.8)/59.2(0.2) \\
\midrule \midrule
& SR & \multirow{5}{*}{Token} & 88.8(0.95) & 81.2(8.4) & 68.8(1.3) & 76.6(1.5)/60.7(1.8) \\ 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Semi Supervised}}}} & LM &   & 88.4(1.87) & 81.4(1.0) & 68.8(1.8) & 76.4(1.3)/60.4(0.7) \\ 
 & RI &  & 88.4(1.45) & 80.3(3.0) & 68.4(2.64) & 76.8(1.2)/60.7(1.1)  \\ 
& RD &  & 88.7(0.5) & 80.5(0.8) & 68.8(1.66) & \textbf{77.1(1.0)/61.2(1.5)}\\ 
 & RS &  & 88.5(1.35) & 80.9(2.2) & 68.7(1.67) & 76.9(1.7)/61.0(1.5) \\ 
& WR &  & 87.7(1.35) & 81.5(1.3) & 68.7(1.2) & 76.5(0.5)/60.6(1.0)\\ \cline{2-7}
& RT & Sentence & 88.7(0.40) & \textbf{81.7(1.0)} & \textbf{69.7(1.06)} & 77.0(1.2)/61.6(1.1) \\  \cmidrule(lr){2-7}
& ADV & \multirow{2}{*}{Hidden} & 88.0(1.04) & 80.4(2.9) & 68.9(1.74) & 76.7(1.5)/60.9(1.2)\\ 
& Cutoff &  & \textbf{88.9(0.25)} & 81.3(4.6) & 69.3(1.76) & 76.7(2.1)/60.7(3.1) \\ 
\bottomrule 
\end{tabular}}
\caption{\small Topic Classification and News Classification results with 100 examples. We report the average results across 3 different random seeds with the 95\% confidence interval and \textbf{bold} the best results.. For PubMed, we report the accuracy and F1 score. } \label{Tab:tc_100}
\end{table*}
